Evaluation of group fairness measures in student performance prediction problems

Predicting students' academic performance is one of the key tasks of educational data mining (EDM). Traditionally, the high forecasting quality of such models was deemed critical. More recently, the issues of fairness and discrimination w.r.t. protected attributes, such as gender or race, have gained attention. Although there are several fairness-aware learning approaches in EDM, a comparative evaluation of these measures is still missing. In this paper, we evaluate different group fairness measures for student performance prediction problems on various educational datasets and fairness-aware learning models. Our study shows that the choice of the fairness measure is important, likewise for the choice of the grade threshold.

==> backup.tex <==
\begin{table}[!h]
\centering
\caption{Student-Math: performance of predictive models}\label{tbl:student_performance_mat}
\begin{tabular}{lcccccc}
\hline
\textbf{Measures} &  
\multicolumn{1}{c}{\textbf{\phantom{aa}DT\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}NB\phantom{aa}}} &
\multicolumn{1}{c}{\textbf{\phantom{aa}MLP\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}RF\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}SVM\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{Adafair}}\\ \hline
Accuracy            & 0.8824 & 0.8487 & 0.9328 & 0.8992 & 0.8739 & 0.9244\\
Balanced accuracy   & 0.8760 & 0.8204 & 0.9251 & 0.8937 & 0.8571 & 0.9343\\
Statistical parity  & 0.1540 & 0.0825 & 0.1868 & 0.1877 & 0.1687 & 0.1402\\
Equal opportunity   & 0.0015 & 0.0169 & 0.0407 & 0.0253 & 0.0492 & 0.0338\\
Equalized odds      & 0.1010 & 0.0871 & 0.1245 & 0.1618 & 0.1271 & 0.0708\\
Predictive parity   & 0.0015 & 0.1257 & 0.0037 & 0.0264 & 0.0404 & 0.0357\\
Predictive equality & 0.0994 & 0.0702 & 0.0838 & 0.1364 & 0.0780 & 0.0370\\
Treatment equality  & 0.0    &-0.1778 & 0.6667 & 0.75   & 0.2    &$N/A$ \\
ABROCA              & 0.0489 & 0.0173 & 0.0228 & 0.0118 & 0.0097 & 0.0354\\
\hline
\end{tabular}
\end{table}

\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{DT.student-mat.abroca.pdf}
    \caption{DT}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{NB.student-mat.abroca.pdf}
    \caption{NB}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{MLP.student-mat.abroca.pdf}
    \caption{MLP}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RF.student-mat.abroca.pdf}
    \caption{RF}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{SVM.student-mat.abroca.pdf}
    \caption{SVM}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Ada.student-mat.abroca.pdf}
    \caption{Adafair}
\end{subfigure}
\caption{Student-Math: ABROCA slice plots}
\label{fig:student_mat_abroca}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experimental results}
\label{subsec:results}
\textbf{Law school dataset.} The detailed results are presented in Table \ref{tbl:law_school}. AdaFair is the best predictive model w.r.t. fairness measures, although its balanced accuracy is significantly lower than that of other models. Besides, the fairness measures show quite large variation across the classification methods, as demonstrated in Fig. \ref{fig:Variation_measures}-a. Furthermore, the shape and position of the ROC curves, as visualized in Fig. \ref{fig:law_school_abroca}, have been changed across the predictive models, which indicates the change in the performance of models w.r.t. each value in the protected attribute.

\begin{table}[!h]
\centering
\caption{Law school: performance of predictive models}\label{tbl:law_school}
\begin{tabular}{lccccccc}
\hline
\textbf{Measures} &  
\multicolumn{1}{c}{\textbf{\phantom{a}DT\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{a}NB\phantom{aa}}} &
\multicolumn{1}{c}{\textbf{\phantom{a}MLP\phantom{aa}}} & 
%\multicolumn{1}{c}{\textbf{\phantom{a}RF\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{a}SVM}} &
\multicolumn{1}{c}{\textbf{\phantom{a}Agarwal's\phantom}} &
\multicolumn{1}{c}{\textbf{AdaFair}}\\ \hline
Accuracy            & 0.8458 & 0.8191 & \textbf{0.9042} & 0.9027 & 0.8926 & 0.8921\\
Balanced accuracy   & 0.6301 & \textbf{0.7784} & 0.6596 & 0.6072 & 0.5029 & 0.5\\
Statistical parity  & 0.1999 & 0.5250 & 0.2367 & 0.1795 & 0.0052 & \textbf{0.0}\\
Equal opportunity   & 0.1557 & 0.4665 & 0.1237 & 0.0881 & 0.0014 & \textbf{0.0}\\
Equalized odds      & 0.3253 & 0.8105 & 0.5501 & 0.4606 & 0.0169 & \textbf{0.0}\\
Predictive parity   & 0.1424 & \textbf{0.0130} & 0.0754 & 0.1058 & 0.1857 & 0.1885\\
Predictive equality & 0.1696 & 0.3440 & 0.4265 & 0.3725 & 0.0154 & \textbf{0.0} \\
Treatment equality  &-0.0667 & 22.440 & 0.7770 & 0.4106 & 0.0039 & \textbf{0.0} \\
ABROCA              & 0.0336 & \textbf{0.0316} & 0.0336 & 0.0365 & 0.0833 & 0.0822\\
\hline
\end{tabular}
\end{table}

\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{DT.law.abroca.pdf}
    \caption{DT}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{NB.law.abroca.pdf}
    \caption{NB}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{MLP.law.abroca.pdf}
    \caption{MLP}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RF.law.abroca.pdf}
    \caption{RF}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{SVM.law.abroca.pdf}
    \caption{SVM}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Ada.law.abroca.pdf}
    \caption{AdaFair}
\end{subfigure}
\caption{Law school: ABROCA slice plots}
\label{fig:law_school_abroca}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%
\textbf{PISA dataset.}
\label{subsubsec:pisa}
The interesting point is SVM and DT show their superiority in terms of fairness measures, although AdaFair still has very good results on these metrics (Fig. \ref{fig:pisa_abroca} and Table \ref{tbl:pisa}). Furthermore, fairness measures have the least variability on this dataset, as shown in Fig. \ref{fig:Variation_measures}-b.
\begin{table}[!h]
\centering
\caption{PISA: performance of predictive models}\label{tbl:pisa}
\begin{tabular}{lcccccc}
\hline
\textbf{Measures} &  
\multicolumn{1}{c}{\textbf{\phantom{aa}DT\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}NB\phantom{aa}}} &
\multicolumn{1}{c}{\textbf{\phantom{aa}MLP\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}RF\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}SVM\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{AdaFair}}\\ \hline
Accuracy            & 0.6360  & 0.6624  & 0.6526  & \textbf{0.7211}  & 0.6096 & 0.6810\\
Balanced accuracy   & 0.6224  & 0.6379  & 0.5732  & \textbf{0.6888}  & 0.5026 & 0.6130\\
Statistical parity  & -0.0200 & -0.0316 & -0.0771 & -0.0885 & \textbf{-0.0022}&-0.0573\\
Equal opportunity   & \textbf{0.0019}  & 0.0262  & 0.0330  & 0.0327  & 0.0043 & 0.0164\\
Equalized odds      & 0.0165  & 0.0709  & 0.1398  & 0.1041  & \textbf{0.0068} & 0.0752\\
Predictive parity   & 0.1012  & 0.0683  & 0.0826  & \textbf{0.0668}  & 0.1108 & 0.0868\\
Predictive equality & 0.0146  & 0.0446  & 0.1067  & 0.0714  & \textbf{0.0024} & 0.0588\\
Treatment equality  & 0.5642  & 0.3855  & -0.0251 & 0.0587  & \textbf{-0.0033}& 0.0260\\
ABROCA              & \textbf{0.0070}  & 0.0330  & 0.0223  & 0.0173  & 0.0844 & 0.0216\\
\hline
\end{tabular}
\vspace{-10pt}
\end{table}

\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{DT.pisa.abroca.pdf}
    \caption{DT}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{NB.pisa.abroca.pdf}
    \caption{NB}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{MLP.pisa.abroca.pdf}
    \caption{MLP}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RF.pisa.abroca.pdf}
    \caption{RF}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{SVM.pisa.abroca.pdf}
    \caption{SVM}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Ada.pisa.abroca.pdf}
    \caption{AdaFair}
\end{subfigure}
\caption{PISA: ABROCA slice plots}
\vspace{-10pt}
\label{fig:pisa_abroca}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Student academics performance dataset}.
\label{subsubsec:student_academics}
The AdaFair outperforms other models w.r.t. fairness measures, however, the balanced accuracy is decreased considerably (Table \ref{tbl:student_academic}). Besides, all fairness measures have significant variation across predictive models (Fig. \ref{fig:student_academics_abroca} and \ref{fig:Variation_measures}-c).
\begin{table}[!hb]
\centering
\caption{Student academics: performance of predictive models}\label{tbl:student_academic}
\begin{tabular}{lcccccc}
\hline
\textbf{Measures} &  
\multicolumn{1}{c}{\textbf{\phantom{aa}DT\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}NB\phantom{aa}}} &
\multicolumn{1}{c}{\textbf{\phantom{aa}MLP\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}RF\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}SVM\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{AdaFair}}\\ \hline
Accuracy            & 0.7750  & 0.8750  & 0.8750 & \textbf{0.9250} & \textbf{0.9250} & 0.9\\
Balanced accuracy   & 0.6528  & \textbf{0.8194}  & \textbf{0.8194} & 0.6250 & 0.6250 & 0.5\\
Statistical parity  & -0.1278 &-0.1328  &-0.1328 &-0.0476 & 0.0526 & \textbf{0.0}\\
Equal opportunity   & 0.1455  & 0.0991  & 0.2105 & 0.0    & 0.0    & \textbf{0.0}\\
Equalized odds      & 0.1455  & 0.5991  & 0.7105 & 0.5    & 0.5    & \textbf{0.0}\\
Predictive parity   & \textbf{0.0042}  & 0.0588  & 0.0625 & 0.0552 & 0.0397 & 0.01\\
Predictive equality & 0.0     & 0.5     & 0.5    & 0.5    & 0.5    & \textbf{0.0}\\
Treatment equality  & -3.0    &$N/A$    & $N/A$  & 0.0    & 0.0    & \textbf{0.0}\\
ABROCA              & 0.0728  & 0.2059  & 0.1316 & 0.0588 & 0.1285 & \textbf{0.0372}\\
\hline
\end{tabular}
\vspace{-10pt}
\end{table}

\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{DT.student-academics.abroca.pdf}
    \caption{DT}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{NB.student-academics.abroca.pdf}
    \caption{NB}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{MLP.student-academics.abroca.pdf}
    \caption{MLP}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RF.student-academics.abroca.pdf}
    \caption{RF}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{SVM.student-academics.abroca.pdf}
    \caption{SVM}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Ada.student-academics.abroca.pdf}
    \caption{AdaFair}
\end{subfigure}
\caption{Student academics: ABROCA slice plots}
\vspace{-10pt}
\label{fig:student_academics_abroca}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Student performance dataset}.
\label{subsubsec:student}
In general, all models show good accuracy (balanced accuracy) on predicting students' performance (Table \ref{tbl:student_performance_por}). MLP and AdaFair models fairly guarantee the fairness of results on most measures. Besides, the values of fairness measures also do not vary significantly across predictive models (Fig. \ref{fig:Variation_measures}-d), although the ABROCA slices are quite different in shape (Fig. \ref{fig:student_por_abroca}).
\begin{table}[!h]
\centering
\caption{Student performance: performance of predictive models}\label{tbl:student_performance_por}
\begin{tabular}{lcccccc}
\hline
\textbf{Measures} &  
\multicolumn{1}{c}{\textbf{\phantom{aa}DT\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}NB\phantom{aa}}} &
\multicolumn{1}{c}{\textbf{\phantom{aa}MLP\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}RF\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}SVM\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{AdaFair}}\\ \hline
Accuracy            & 0.9333 & 0.8974 & 0.9077 & 0.9385 & 0.9231 & \textbf{0.9487}\\
Balanced accuracy   & \textbf{0.8639} & 0.8595 & 0.7840 & 0.8343 & 0.7441 & 0.8240\\
Statistical parity  &-0.0382 &-0.0509 &-0.0630 &\textbf{-0.0142} & 0.0151 &-0.0255\\
Equal opportunity   & 0.0125 & 0.0174 & 0.03   & 0.0150 & 0.0183 & \textbf{0.0092} \\
Equalized odds      & 0.1316 & 0.2198 & \textbf{0.1252} & 0.4317 & 0.3279 & 0.1877\\
Predictive parity   & \textbf{0.0456} & 0.0591 & 0.0601 & 0.0984 & 0.0944 & 0.0639\\
Predictive equality & 0.1190 & 0.2024 & \textbf{0.0952} & 0.4167 & 0.3095 & 0.1786\\
Treatment equality  & 2.0    & 7.5    & \textbf{0.3333} & 1.7143 & 0.5    & \textbf{0.3333}\\
ABROCA              & 0.0575 & 0.0686 & 0.0683 & 0.0544 & \textbf{0.0231} & 0.0887\\
\hline
\end{tabular}

\end{table}

\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{DT.student-por.abroca.pdf}
    \caption{DT}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{NB.student-por.abroca.pdf}
    \caption{NB}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{MLP.student-por.abroca.pdf}
    \caption{MLP}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RF.student-por.abroca.pdf}
    \caption{RF}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{SVM.student-por.abroca.pdf}
    \caption{SVM}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Ada.student-por.abroca.pdf}
    \caption{AdaFair}
\end{subfigure}
\caption{Student performance: ABROCA slice plots}
\vspace{-5pt}
\label{fig:student_por_abroca}
\vspace{-10pt}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{xAPI-Edu-Data dataset} 
\label{subsubsec:xAPI-Edu-Data}
This is a surprising dataset because the traditional classification methods show a better performance not only in terms of accuracy/balanced accuracy measures but also w.r.t. fairness measures (Table \ref{tbl:xAPI-Edu-Data}). In addition, variation in the values of fairness measures across the predictive models is not significant, as shown in Fig. \ref{fig:Variation_measures}-e, except the ABROCA measure with a noticeable change in the shape (Fig. \ref{fig:xAPI-Edu-Data_abroca}). 

Regarding the \emph{treatment equality} measure, this measure is completely different from all other measures in the range of values, which is visualized in Fig. \ref{fig:Variation_measures}-f. On the \emph{PISA} datasets, this TE measure shows the best values across predicted models, followed by \emph{Law school} and \emph{Student Academics} datasets.

\begin{table}[!h]
\centering
\caption{xAPI-Edu-Data: performance of predictive models}\label{tbl:xAPI-Edu-Data}
\begin{tabular}{lcccccc}
\hline
\textbf{Measures} &  
\multicolumn{1}{c}{\textbf{\phantom{aa}DT\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}NB\phantom{aa}}} &
\multicolumn{1}{c}{\textbf{\phantom{aa}MLP\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}RF\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{\phantom{aa}SVM\phantom{aa}}} & 
\multicolumn{1}{c}{\textbf{AdaFair}}\\ \hline
Accuracy            & 0.8333 & 0.8750 & 0.8750 & \textbf{0.9236} & 0.8611 & 0.8056\\
Balanced accuracy   & 0.8    & 0.8970 & 0.8545 & \textbf{0.9202} & 0.8505 & 0.8162\\
Statistical parity  &\textbf{-0.1274} &-0.2608 &-0.2112 &-0.2106 &-0.2209 &-0.2292 \\
Equal opportunity   & 0.0282 & 0.0974 & 0.0654 & \textbf{0.0102} & 0.0308 & 0.0538\\
Equalized odds      & \textbf{0.1329} & 0.1954 & 0.1262 & 0.2062 & 0.2706 & 0.3207\\
Predictive parity   & 0.0752 & 0.0074 & 0.0654 & 0.0181 & 0.0088 & \textbf{0.0057}\\
Predictive equality & \textbf{0.1047} & 0.0980 & 0.0608 & 0.1959 & 0.2399 & 0.2669\\
Treatment equality  & 1.0667 & -8.0   & \textbf{0.0}    & -0.5   &-0.2667 & -1.1667\\
ABROCA              & 0.0665 & \textbf{0.0216} & 0.0263 & 0.0282 & 0.0796 & 0.1065\\
\hline
\end{tabular}
\vspace{-10pt}
\end{table}

\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{DT.xAPI-Edu-Data.abroca.pdf}
    \caption{DT}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{NB.xAPI-Edu-Data.abroca.pdf}
    \caption{NB}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{MLP.xAPI-Edu-Data.abroca.pdf}
    \caption{MLP}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RF.xAPI-Edu-Data.abroca.pdf}
    \caption{RF}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{SVM.xAPI-Edu-Data.abroca.pdf}
    \caption{SVM}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Ada.xAPI-Edu-Data.abroca.pdf}
    \caption{AdaFair}
\end{subfigure}
\caption{xAPI-Edu-Data: ABROCA slice plots.}
\vspace{-10pt}
\label{fig:xAPI-Edu-Data_abroca}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{boxplot.law.pdf}
    \caption{Law school}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{boxplot.pisa.pdf}
    \caption{PISA}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{boxplot.student-academic.pdf}
    \caption{Student academic}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{boxplot.student-por.pdf}
    \caption{Student performance}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{boxplot.xAPI-Edu-Data.pdf}
    \caption{xAPI-Edu-Data}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{boxplot.TE.pdf}
    \caption{TE measure}
\end{subfigure}
\caption{Variation of fairness measures}%\textsuperscript{*}}
% \small\textsuperscript{*} We use the abbreviations of the fairness measures and datasets in this figure.
\vspace{-20pt}
\label{fig:Variation_measures}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-5pt}
\subsection{Effect of varying grade threshold on fairness}
\label{subsec:threshold}
Grade thresholds are often chosen as a basis for determining whether a candidate passes or fails an exam. In the student performance dataset, 10 (out of 20) is selected as the grade threshold \cite{cortez2008using,lequy2022survey}. However, the selection of a threshold can affect fairness of the predictive models, as shown in the IPUMS Adult dataset \cite{ding2021retiring}. Hence, we investigate the effect of grade threshold on fairness by varying the threshold in a range of [4, 16], corresponding to 25\% to 75\% of the maximum grade (20). The results in Fig. \ref{fig:threshold} show that all fairness measures are affected by the grade threshold. When the grade threshold is gradually increased, the predictive model tends to be more fair (shown on the measures: equalized odds, predictive equality and ABROCA). The opposite trend is observed on remaining measures (except treatment equality measure). Regarding the balanced accuracy, 2 models (DT and AdaFair) tend to predict more accurately. The NB model has a decreasing accuracy after the threshold is increased.
\begin{figure*}[!h]
\centering
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Accuracy.pdf}
    \caption{Accuracy}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Balanced accuracy.pdf}
    \caption{Balanced accuracy}
\end{subfigure}    
\hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Statistical parity.pdf}
    \caption{Statistical parity}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Equal opportunity.pdf}
    \caption{Equal opportunity}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Equalized odds.pdf}
    \caption{Equalized odds}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Predictive parity.pdf}
    \caption{Predictive parity}
\end{subfigure}
\bigskip
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Predictive equality.pdf}
    \caption{Predictive equality}
\end{subfigure}
\hfill
\vspace{-5pt}
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.Treatment equality.pdf}
    \caption{Treatment equality}
\end{subfigure}
\vspace{-5pt}
 \hfill
\begin{subfigure}{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Thres.ABROCA.pdf}
    \caption{ABROCA}
\end{subfigure}
\caption{Accuracy and fairness interventions with varying grade threshold on Student performance dataset (Decision Tree method).}
\vspace{-10pt}
\label{fig:threshold}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%
